A Localized Reality Appears To Underpin Quantum Circuits

Although entangled state vectors cannot be described in terms of classically realistic variables, localized in space and time, any given entanglement experiment can be built from basic quantum circuit components with well-defined locations. By analyzing the (local) weak values for any given run of a quantum circuit, we present evidence for a localized account of any circuit's behavior. Specifically, even if the state is massively entangled, the weak values are found to evolve only when they pass through a local circuit element. They otherwise remain constant and do not evolve when other qubits pass through their circuit elements. A further surprise is found when two qubits are brought together in an exchange interaction, as their weak values then evolve according to a simple classical equation. The weak values are subject to both past and future constraints, so they can only be determined by considering the entire circuit "all-at-once", as in action principles. In the context of a few basic quantum gates, we show how an all-at-once model of a complete circuit could generate weak values without using state vectors as an intermediate step. Since these gates comprise a universal quantum gate set, this lends support to the claim that any quantum circuit can plausibly be underpinned by localized variables, providing a realistic, lower-level account of generic quantum systems.

==> weak_value_paper_eq_14_proff.tex <==
Adding eqs. (14) and (15) based on the limit definition of the derivative, we get:
\\
\begin{align*}
    U_{ex}(\Delta \tau)^\dagger A U_{ex}(\Delta \tau) -2A + U_{ex}(\Delta \tau) A U_{ex}(\Delta \tau)^\dagger + \\
    U_{ex}(\Delta \tau)^\dagger B U_{ex}(\Delta \tau) -2B + U_{ex}(\Delta \tau) B U_{ex}(\Delta \tau)^\dagger = 0
    \\
     U_{ex}(\Delta \tau)^\dagger (A + B) U_{ex}(\Delta \tau) + U_{ex}(\Delta \tau) (A + B) U_{ex}(\Delta \tau)^\dagger = 2(A + B) \tag{**}
\end{align*}
\\
Subtracting eq. (15) from (14) based on the limit definition of the derivative, we get:
\\
\begin{align*}
    U_{ex}^\dagger(\Delta \tau) A U_{ex}(\Delta \tau) -2A + U_{ex}(\Delta \tau) A U_{ex}(\Delta \tau)^\dagger -\\
    - U_{ex}(\Delta \tau)^\dagger B U_{ex}(\Delta \tau) +2B - U_{ex}(\Delta \tau) B U_{ex}(\Delta \tau)^\dagger = 2(B - A)
    \\
     U_{ex}(\Delta \tau)^\dagger (A - B) U_{ex}(\Delta \tau) + U_{ex}(\Delta \tau) (A - B) U_{ex}(\Delta \tau)^\dagger = 0 \tag{***}
\end{align*}
\\
Adding $(**)$ and $(***)$, we get:
\begin{align*}
    U_{ex}^\dagger(\Delta \tau) A U_{ex}(\Delta \tau) + U_{ex}(\Delta \tau) A U_{ex}^\dagger(\Delta \tau) = A + B
\end{align*}
Plugging this result into $(*)$:
\begin{align*}
    U_{ex}^\dagger(\Delta \tau) A U_{ex}(\Delta \tau) -2A + U_{ex}(\Delta \tau) A U_{ex}^\dagger(\Delta \tau)  = A + B - 2A = B - A
\end{align*}
Thus, LHS of eq. (14) becomes:
\begin{align*}
\frac{d^2 w_a}{d \tau ^2} = \frac{\langle f|U_{ex}(\alpha - \tau)[U_{ex}^\dagger(\Delta \tau) A U_{ex}(\Delta \tau) -2A + U_{ex}(\Delta \tau) A U_{ex}^\dagger(\Delta \tau)]U_{ex}(\tau)| i \rangle}{(\Delta \tau)^2} \\
= \frac{\langle f|U_{ex}(\alpha - \tau)[B-A]U_{ex}(\tau)| i \rangle}{(\Delta \tau)^2} \\
= \frac{w_b - w_a}{(\Delta \tau)^2} \propto \frac{\pi^2}{2}(w_b - w_a)
\end{align*}
It can be shown that for $\Delta \tau = \frac{\sqrt{2}}{\pi}$, $U_{ex}^{n}(\Delta \tau) \longrightarrow SWAP$ as $n \rightarrow \infty$.
It can also be shown that for $\Delta \tau$ values such as $\frac{2}{\pi}$ or $\frac{1}{\pi}$ $U_{ex}(\Delta \tau)$ diverges from the SWAP form as $n \rightarrow \infty$.\\
Thus, $\Delta \tau = \frac{\sqrt{2}}{\pi}$ is a good choice in the limit of $n \rightarrow \infty$.
Moving $\Delta \tau^2$ to RHS of $(*)$, we recover the $\frac{\pi^2}{2}$ factor.
\qedhere
\\
\\
We can work out the commutation relation between $A$, $B$ and $U_{ex}(\Delta \tau)$: $[U_{ex}(\Delta \tau), A] = [B, U_{ex}(\Delta \tau)]$, which holds true for all Pauli matrices. Thus, we can expand the left side of eq. (14):\\
\begin{align*}
[U_{ex}(\Delta\tau), A] = U_{ex}(\Delta\tau)A - AU_{ex}(\Delta\tau) = [B, U_{ex}(\Delta\tau)]\\
\\
U_{ex}(\Delta\tau) A U_{ex}^{\dagger}(\Delta\tau) = \Big( [B, U_{ex}(\Delta\tau)] + AU_{ex}(\Delta\tau) \Big) U_{ex}^{\dagger}(\Delta\tau)\\
= \Big(B U_{ex}(\Delta\tau) - U_{ex}(\Delta\tau) B + A U_{ex}(\Delta\tau)\Big) U_{ex}^{\dagger}(\Delta\tau)\\
= B + U_{ex}(\Delta\tau) B U_{ex}^{\dagger}(\Delta\tau) + A\\
\\
U_{ex}^{\dagger}(\Delta\tau) A U_{ex}(\Delta\tau) = U_{ex}^{\dagger}(\Delta\tau) \Big(U_{ex}(\Delta\tau) A - [B, U_{ex}(\Delta\tau)]\Big)\\
= U_{ex}^{\dagger}(\Delta\tau) \Big(U_{ex}(\Delta\tau) A - B U_{ex}(\Delta\tau) + U_{ex}(\Delta\tau) B \Big)\\
= A + U_{ex}^{\dagger}(\Delta\tau) B U_{ex}(\Delta\tau) + B
\end{align*}
Thus:
\[
U_{ex}(\Delta \tau)^\dagger A U_{ex}(\Delta \tau) -2A + U_{ex}(\Delta \tau) A U_{ex}(\Delta \tau)^\dagger = - \Big(U_{ex}^{\dagger}(\Delta\tau) B U_{ex}(\Delta\tau) - 2B + U_{ex}(\Delta\tau) B U_{ex}^{\dagger}(\Delta\tau) \Big)
\]
which is true since $\frac{d^2 w_a}{d \tau^2} = - \frac{d^2 w_b}{d \tau^2}$.\\
\\
\end{proof}

\begin{proof}
2. Proof for equations 14 and 15\\
Given the Hamiltonian:
\begin{align*}
H = \frac{\pi}{4} \Big ( \sigma_x \otimes \sigma_x + \sigma_y \otimes \sigma_y + \sigma_z \otimes \sigma_z - I \otimes I \Big) = \frac{\pi}{2}H'
\end{align*}

and writing the unitary evolution matrix $U_{ex}$ using $H$, we get:
\begin{align*}
U_{ex}[\tau] = e^{-i H \tau} = e^{-i \frac{\pi}{2} H' \tau}\\
U_{ex}[\alpha - \tau] = e^{-i H (\alpha - \tau)} = e^{-i \frac{\pi}{2} H' (\alpha - \tau)}
\end{align*}

The derivatives of $U_{ex}$ based on the exponential form are:
\begin{align*}
\frac{d}{d\tau} U_{ex}[\tau] = -iH e^{-iH\tau} = -\frac{i\pi}{2}H' e^{- \frac{i\pi}{2} H'\tau}\\
\frac{d^2}{d\tau^2} U_{ex}[\tau] = (-iH)^2 e^{-iH\tau} = -\frac{\pi^2}{4}H'^2 e^{-\frac{i \pi}{2}H'\tau} \\
\frac{d}{d\tau} U_{ex}[\alpha - \tau] = iH U_{ex}[\alpha - \tau] = \frac{i \pi}{2} H' U_{ex}[\alpha - \tau] \\
\frac{d^2}{d\tau^2} U_{ex}[\alpha - \tau] = -H^2 U_{ex}[\alpha - \tau] = -\frac{\pi^2}{4} H'^2 U_{ex}[\alpha - \tau]
\end{align*}

Taking the second derivative of $w_a$, we get:
\begin{align*}
\frac{d^2}{d\tau^2} s_a(\tau) = \frac{1}{D} \langle \psi_f | (-\frac{\pi^2}{4} H'^2) U_{ex}[\alpha - \tau](\sigma \otimes I) U_{ex}[\tau] \\
    + 2(-i\frac{\pi}{2}H') U_{ex}[\alpha - \tau](\sigma \otimes I)(i\frac{\pi}{2}H') U_{ex}[\tau] \\
    + U_{ex}[\alpha - \tau](\sigma \otimes I)(-\frac{\pi^2}{4} H'^2) U_{ex}[\tau] | \psi_i \rangle\\
\\
\propto \frac{\pi^2}{4} \Big(-H'^2 U_{ex}[\alpha - \tau](\sigma \otimes I) U_{ex}[\tau] \\
    + 2H' U_{ex}[\alpha - \tau](\sigma \otimes I)H' U_{ex}[\tau] \\
    - U_{ex}[\alpha - \tau](\sigma \otimes I) H'^2 U_{ex}[\tau] \Big)\\
\\
-H^2 U_{ex}[\alpha - \tau](\sigma \otimes I) U_{ex}[\tau] + 2H U_{ex}[\alpha - \tau](\sigma \otimes I)H U_{ex}[\tau] - U_{ex}[\alpha - \tau](\sigma \otimes I) H^2 U_{ex}[\tau] = \\
H^2 U_{ex}[\alpha - \tau](I \otimes \sigma) U_{ex}[\tau] - 2H U_{ex}[\alpha - \tau](\sigma \otimes I)H U_{ex}[\tau] + U_{ex}[\alpha - \tau](I \otimes \sigma) H^2 U_{ex}[\tau] \Leftrightarrow \\
\\
-H^2 U_{ex}[\alpha - \tau](\sigma \otimes I) + 2H U_{ex}[\alpha - \tau](\sigma \otimes I)H - U_{ex}[\alpha - \tau](\sigma \otimes I) H^2 = \\
H^2 U_{ex}[\alpha - \tau](I \otimes \sigma) - 2H U_{ex}[\alpha - \tau](I \otimes \sigma)H + U_{ex}[\alpha - \tau](I \otimes \sigma) H^2
\end{align*}
If $H$ and $H^2$ commute with $U_{ex}[\alpha - \tau]$ (and they should since $U_{ex}$ is a Taylor expansion of $H$ matrices), then:
\begin{align*}
-H^2 (\sigma \otimes I) + 2H (\sigma \otimes I)H - (\sigma \otimes I) H^2 = \\
H^2 (I \otimes \sigma) - 2H (I \otimes \sigma)H + (I \otimes \sigma) H^2\\
\\
H^2 (\sigma \otimes I) + (\sigma \otimes I) H^2 + H^2 (I \otimes \sigma) + (I \otimes \sigma) H^2 = 2H (\sigma \otimes I)H + 2H (I \otimes \sigma)H\\
\end{align*}
Multiplying by $H^{-1}$ to the left and right:
\begin{align*}
    H A H^{-1} + H^{-1} A H + H B H^{-1} + H^{-1} B H = 2(A + B)\\
\begin{pmatrix}
0 & 0 & 0 & 0 \\
0 & \frac{i \pi \Delta \tau - \frac{\pi^2 \Delta \tau^2}{2}}{2} & \frac{- i \pi \Delta \tau - \frac{\pi^2 \Delta \tau^2}{2}}{2} & 0 \\
0 & \frac{- i \pi \Delta \tau - \frac{\pi^2 \Delta \tau^2}{2}}{2} & \frac{i \pi \Delta \tau - \frac{\pi^2 \Delta \tau^2}{2}}{2} & 0 \\
0 & 0 & 0 & 0
\end{pmatrix}
\end{align*}
\begin{align*}
\begin{pmatrix}
0 & 0 & 0 & 0 \\
0 & 1 & - 1 & 0 \\
0 & - 1 & 1 & 0 \\
0 & 0 & 0 & 0
\end{pmatrix}\\
\begin{pmatrix}
0 & 0 & 0 & 0 \\
0 & 1 +i \frac{\pi \Delta \tau}{2} & - 1 -i \frac{\pi \Delta \tau}{2} & 0 \\
0 & - 1 -i \frac{\pi \Delta \tau}{2} & 1 +i \frac{\pi \Delta \tau}{2} & 0 \\
0 & 0 & 0 & 0
\end{pmatrix} \\

\end{align*}
\begin{align*}
     U_{ex}(\Delta \tau) \approx I + i\frac{\pi \Delta \tau}{2} \Big ( 1 +i \frac{\pi \Delta \tau}{2} \Big)M = I + \left( i \frac{\pi \Delta \tau}{2} - \frac{\pi^2 \Delta \tau^2}{4} \right) \frac{1}{2} \Big ( I - \sigma_x \otimes \sigma_x -\sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z \Big )
\end{align*}
\begin{align*}
A = \left( i \frac{\pi \Delta \tau}{2} - \frac{\pi^2 \Delta \tau^2}{4} \right) \frac{1}{2}\\
\\
 M =  I - \sigma_x \otimes \sigma_x -\sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z\\
 \\
U_{ex}(\Delta \tau) (\sigma_x \otimes I) U_{ex}^\dagger(\Delta \tau) = (\sigma_x \otimes I) + A^\dagger (\sigma_x \otimes I)(I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z) \\ 
+ A (I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z)(\sigma_x \otimes I) \\ 
+ AA^\dagger (I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z)(\sigma_x \otimes I)(I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z)\\
\\
\\
U_{ex}^\dagger (\Delta \tau)(\sigma_x \otimes I) U_{ex}(\Delta \tau) = (\sigma_x \otimes I) 
+ A (\sigma_x \otimes I)(I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z) \\
+ A^\dagger (I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z)(\sigma_x \otimes I) \\
+ AA^\dagger (I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z)(\sigma_x \otimes I)(I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z)\\
\\
\end{align*}
\\
Thus, $U_{ex}^\dagger(\Delta \tau) (\sigma \otimes I) U_{ex}(\Delta \tau) - 2(\sigma \otimes I) + U_{ex}(\Delta \tau) (\sigma \otimes I) U_{ex}^\dagger(\Delta \tau)$ becomes:
\begin{align*}
2AA^\dagger (I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z)(\sigma_x \otimes I)(I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z)+\\
(A + A^\dagger) \Big ((\sigma_x \otimes I)(I - \sigma_x \otimes \sigma_x -\sigma_y \otimes \sigma_y  - \sigma_z \otimes \sigma_z) + \\
+ (I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y  - \sigma_z \otimes \sigma_z)(\sigma_x \otimes I) \Big)\\
\\
A + A^\dagger = \frac{1}{2} \Big ( i \frac{\pi \Delta \tau}{2} - \frac{\pi^2 \Delta \tau^2}{4}  - i \frac{\pi \Delta \tau}{2} - \frac{\pi^2 \Delta \tau^2}{4} \Big) = -\frac{\pi^2 \Delta \tau^2}{4}
\\
AA^\dagger = - \frac{1}{4}(i \frac{\pi \Delta \tau}{2} - \frac{\pi^2 \Delta \tau^2}{4})(i \frac{\pi \Delta \tau}{2} + \frac{\pi^2 \Delta \tau^2}{4}) = \frac{1}{16}\Big (\frac{\pi^4 \Delta \tau^4}{4}  + \pi^2 \Delta \tau^2 \Big )
\end{align*}
First term:
\begin{align*}
    (I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z)(\sigma_x \otimes I)(I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z) = 0
\end{align*}
Second term:
\begin{align*}
    (\sigma_x \otimes I)(I - \sigma_x \otimes \sigma_x -\sigma_y \otimes \sigma_y  - \sigma_z \otimes \sigma_z) + (I - \sigma_x \otimes \sigma_x - \sigma_y \otimes \sigma_y  - \sigma_z \otimes \sigma_z)(\sigma_x \otimes I) = \\
    = 2 \sigma_x \otimes I - 2I \otimes \sigma_x - i \sigma_z \otimes \sigma_y + i \sigma_y \otimes \sigma_z + i \sigma_z \otimes \sigma_y - i \sigma_y \otimes \sigma_z = 2(\sigma_x \otimes I - I \otimes \sigma_x)
\end{align*}
Thus, for the 2nd order expansion in small $\Delta \tau$:
\begin{align*}
    U_{ex}^\dagger(\Delta \tau) (\sigma \otimes I) U_{ex}(\Delta \tau) - 2(\sigma \otimes I) + U_{ex}(\Delta \tau) (\sigma \otimes I) U_{ex}^\dagger(\Delta \tau) = 2(A + A^\dagger)(\sigma_x \otimes I - I \otimes \sigma_x)=\\
    = -\frac{\pi^2 \Delta \tau^2}{4}2(\sigma_x \otimes I - I \otimes \sigma_x)=\frac{\pi^2 \Delta \tau^2}{2}(I \otimes \sigma_x - \sigma_x \otimes I)
\end{align*}

However, if we truncated to 1st order in $\Delta \tau$:
\begin{align*}
    U_{ex}(\Delta \tau) \approx I + i \frac{\pi \Delta \tau}{2} \frac{1}{2} M= I + \Big ( i\frac{\pi \Delta \tau}{4} \Big)  \Big ( I - \sigma_x \otimes \sigma_x -\sigma_y \otimes \sigma_y - \sigma_z \otimes \sigma_z \Big )\\
    \\
     A = i \frac{\pi \Delta \tau}{4}\\    
    \\
    AA^\dagger = \frac{\pi^2 \Delta \tau^2}{16}\\
    \\
    A + A^\dagger = 0
\end{align*}
the approximation fails, since both terms become zero.
      
